Orthogonal Adaptation for Modular Customization of Diffusion Models

Customization techniques for text-to-image models have paved the way for a wide range of previously unattainable applications, enabling the generation of specific concepts across diverse contexts and styles. While existing methods facilitate high-fidelity customization for individual concepts or a limited, pre-defined set of them, they fall short of achieving scalability, where a single model can seamlessly render countless concepts. In this paper, we address a new problem called Modular Customization, with the goal of efficiently merging customized models that were fine-tuned independently for individual concepts. This allows the merged model to jointly synthesize concepts in one image without compromising fidelity or incurring any additional computational costs. To address this problem, we introduce Orthogonal Adaptation, a method designed to encourage the customized models, which do not have access to each other during fine-tuning, to have orthogonal residual weights. This ensures that during inference time, the customized models can be summed with minimal interference. Our proposed method is both simple and versatile, applicable to nearly all optimizable weights in the model architecture. Through an extensive set of quantitative and qualitative evaluations, our method consistently outperforms relevant baselines in terms of efficiency and identity preservation, demonstrating a significant leap toward scalable customization of diffusion models.

==> sec/3_method.tex <==
\section{Preliminary}

\paragraph{Decentralized Multi-Concept Personalization}
In this paper, we are interested in customize text-to-image diffusion models to generate multiple personal concepts in a decentralized, scalable, and efficient way.
Each user is able to create their own customized concepts by defining a set of images $\iI^i = \{I^i_j\}_j$ and a special token $t_i$ that identifies the common concept inside the dataset  $\iI_i$.
Text-to-image customization aims to fine-tune the diffusion model (\ie updating model weights or creating latent word embeddings) to optimize for two objectives:
\begin{enumerate}
    \item using $t_i$ in the caption can generate images that contains concept represented in $\iI_i$, 
    and
    \item preventing the customized model from catastrophic forgetting so the concept in $\iI_i$ can be used together with other vocabularies.
\end{enumerate}

\todo{(Motivate decentralized)}
In addition to the abovementioned requirements for text-to-image customization, users are usually interested in seeing multiple personalized concepts interacting together.
This calls for a text-to-image model that is aware of a set of personalized concepts.
Being able to generate multiple personalized concepts in a single model, however, is challenging.
First, all possible sets of concepts is growing exponentially with respect to the number of personal concepts, which is only going to be an ever-increasing number. 
As a result, it's important for personalized concepts to be merged with interactive speed .
Furthermore, users usually have limited compute at their end (\eg a phone or a personal laptop without SOTA GPUs), which further prevents extensive optimization process as required by many .
\todo{(privacy argument, not sure if it stands) Last, it's hard to preserve user data privacy if every time we want to generate images of two merged concepts required accessing to the original data that personalized the concepts.}

Motivated by such real-world considerations, we propose the decentralized multi-concept personalization setting.
% Our goal is to derive an algorithm to achieve this with decentralized training.
In this setting, each user is fine-tuning the diffusion model for his/her own concepts of interst.
During inference, the user can choose multiple concepts, represented by the fine-tuned weights or word embedding, to create a fused weights or word embedding capable of generating multiple concepts.
The weight fusing process usually do not have access to the dataset used for creating the individual concepts.
The objective is to generate images with multiple concepts efficiently while preserving the two personalization objectives described above.
Please see Figure~\ref{fig:setup} for an illustration of our problem setup.
\input{figures/problem-setup/fig}

\paragraph{Training objectives.}

To fine-tune a diffusion model $\dD$ with initial weights $\theta_o$ to generate a personalized concept, one usually optimize the diffusion training objective using a curated dataset of image-caption pairs $\dD=\{(I_i, c_i)\}_i$:
\begin{align}
    % \label{eq:loss-cus}
    \label{eq:loss-diff}
    \lL_{\text{diff}}(\theta,\dD) = \Ee_{(\xx, \cc)\sim\dD,t,\epsilon}\left[
        \norm{
        \mM_{\theta}\paren{\xx_t, t, \cc} - \xx
        }^2
    \right],
\end{align}
where $x_t = \alpha_t x + \beta_t \epsilon$ is the noisy image created with Gaussian noise $\epsilon\sim\nN(0,I)$ and 
$\alpha_t, \beta_t$ are weights schedules \todo{cite-EDM}.
Prior workds propose several different ways to create the text-image pairs to achieve both the \todo{overfitting} and the \todo{non-forgetting} requirements of personalization.
For example, Dreambooth~\cite{ruiz2023dreambooth} optimize this loss using a dataset containing the images in user defined dataset $\iI$, pairing with the captions using $t_i$ to describe the concept.
Dreambooth also optimizes a regularization loss to preserve the meaning of the word describing the concept's class.
Our formulation can work with different ways to construct the fine-tuning dataset, so we will denote the optimization loss of the $i^{\text{th}}$ concept to be $\lL_i(\theta)$ for convenience.
% This loss makes sure the fine-tuned diffusion model can generate images containing the subject the concept $c_i$ wants to capture while conditioned on the customized caption.

Under this formulation, finding the optimal weights to combine these customized concepts into the same model can be formulated as optimizing for all objectives together:
\begin{align}
    \lL_{\text{merge}}(\theta) = \sum_{i} \lambda_i\lL_i(\theta),
\end{align}
where $\lL_i$ is computed using dataset $\iI_i, c_i$.
However, such optimization can be computationally expensive to run for each possible combination of concepts. 
In the following sections, we will propose a method to customize the weights for the diffusion models (\ie finding $\theta_i$ and $c_i$) that can be combined together without any additional fine-tuning/optimization.


\section{Method}
\label{sec:method}

\todo{Quick outline of section}

\subsection{Orthogonal Gradient Descent}
Ideally, if the user has access to all concepts and images to be customized, it should try to optimize the loss $\lL_{\text{merge}}$ using gradient descent:
\begin{align}
    \theta_i^{t+1} \leftarrow \theta_i^t - \alpha \sum_j \lambda_j \nabla_\theta\lL_j(\theta_i^t),
\end{align}
where $\theta_i^t$ denotes the parameters for the $i^{th}$ concept at time step $t$ and $\alpha$ is the learning rate.
Unfortunately, this is not achievable since the data to compute gradients for loss $\lL_j$ is not available when $i\neq j$ from the view of a particular user who only has access to dataset $\iI_i$ and the token $t_i$.
Instead, one can only conduct the update using gradient for $\lL_i$:
\begin{align}
    \theta_i^{t+1} \leftarrow \theta_i^t - \alpha \nabla_\theta\lL_i(\theta_i^t).
\end{align}
But these gradient directions can potentially increase the customization loss $\lL_j$ when $i\neq j$.

% \guandao{maybe going straight to the orthogonal argument without this? I think OGD doesn't really add much.} \po{I think starting with OGD makes sense, it motivates the case for orthogonality. We can maybe make this brief.}
Similar issues arise in continual-learning/federate-learning, where one would like to fine-tune a model optimized for task A for task B without access to data of task A \todo{cite}.
One way to alleviate such an issue is to conduct updates at the direction that won't increase the loss $\lL_j$ as much.
This can be achieved by projecting out the updating direction parallel to the gradient direction of $\lL_j$.
The intuition is that orthogonal direction to the gradient of $\lL_j$ will affect the loss $\lL_j$ the least locally.
Specifically, the projected updating rule is:
\begin{align}
    \label{eq:ogd}
    \theta_i^{t+1} 
    \leftarrow 
    \theta_i^t - \alpha \paren{
        \gg_i^t - \sum_j \operatorname{proj}_j\paren{\gg_i^t}
    },
\end{align}
where $\gg_i^t$ is the gradient step, usually chosen to be $\nabla \lL_i(\theta_i^t)$.
The operator $\operatorname{proj}_j(\gg) = \aa_j^T\gg\aa_j\norm{\aa_j}^{-1}$ projects the gradient $\gg$ onto the direction that increase the loss $\lL_j$ the most: $\aa_j$.
While the ideal choice for $\aa_j$ is the gradient evaluated at the current time step: $\nabla_\theta \lL_j(\theta_i^t)$, this cannot be achieved without knowing the data.
\todo{cite-osgd} approximates $\nabla_\theta \lL_j(\theta_i^t)$ using gradient evaluated at the the parameter that minimized $\lL_j$ at each task: $\aa_j = \nabla_\theta \lL_j(\theta_j^*)$.
This way, one only needs access to this set of gradients $\{\aa_j\}_j$, without accessing the dataset for individual concepts.
\guandao{With these updating steps, one can guarantee that $\theta_i^* - \theta_i^0$ is orthogonal to $\aa_j$ for all $j$'s. 
This suggests that $\theta_i^*$ only moves along the direction that does not increase other losses $\lL_j, i\neq j$ as much.
}

Directly applying orthogonal gradient descent to our setting requires knowing the set of concepts we would like to combine during training time.
Such information, however, is not available in the decentralized multi-concept customization setting, where users only have access to their own concept during training time.
% This may require additional fine-tuning steps during merging, hurting the scalability of the method.

\subsection{Orthogonal Constrained Gradient Descent}

Is there a way to apply the intuition of orthogonal gradient descent to the decentralized personalization setting, where the optimization can only compute losses using the dataset of the current concept?
One way to achieve this is to enforce that the gradient direction for one concept, $\nabla \lL_i$, is always orthogonal to that of a different concept: $\nabla \lL_j$.
If this is the case, updating along the direction $\nabla \lL_i$ (as what each individual user would do) will walk among the direction orthogonal to that would increase the loss of $\lL_j$.
To achieve this, we propose to parameterize the model updates in the following way:
\begin{align}
    \theta_i = \theta_o + B_i\Theta_i,
\end{align}
where $\theta_i\in \Re^D$ contains all trainable parameters of the diffusion model, 
$\theta_o$ is the original trainable parameters where we are fine-tuning from, 
$\Theta_i \in \Re^d$ is the constrained set of trainable parameters we will fine-tune(with $d<D$), 
and $B_i\in \Re^{D\times d}$ is a basis matrix that project these parameters back to the original space of $\Re^d$.
% With such parameterization, 
We will update the parameter using the following rule during training (freezing $B_i$ and $\theta_o$):
\begin{equation}\label{eq:projected-sgd}
\begin{aligned}
    \Theta_i^{t+1} &\leftarrow \Theta_i^t - \alpha_t \nabla_\Theta \lL_i(\theta_i^t) \\
    \theta_i^{t+1} &= \theta_o + B_i\Theta_i^{t+1}
\end{aligned},
\end{equation}
where $\Theta_i^0$ is initialized to be \todo{zero} and $B_i$ is freezed during training.
With this updating rule, updating direction of the $i^{\text{th}}$ concept, $\theta_i^{t+1}-\theta_i^t$, is orthogonal to that of the $j^{\text{th}}$, $\theta_j^{t'+1}-\theta_j^{t'
}$, as long as $B_i^TB_j =0$ for all $i \neq j$:
\begin{align*}
(\theta_i^{t+1}-\theta_i^t)^T(\theta_j^{t'+1}-\theta_j^{t'})
% &\propto  (B_i\nabla_{\Theta_i}\lL_i)^T(B_j\nabla_{\Theta_j} \lL_jh)  \\
&\propto \nabla_{\Theta_i}\lL_i^T\cancelto{0}{B_i^TB_j}\nabla_{\Theta_j} \lL_j.
\end{align*}

\paragraph{Why is the constrained optimization expressive enough?}
Since we are optimizing in a linear subspace instead of the full parameter space, it's important to assess whether these subspace are expressive enough to optimize the customization loss $\lL_i$.
Fortunately, diffusion models usually are highly over-parameterized with millions/billion of parameters.
Prior works have shown that even fine-tuning a subspace of such parameters can be expressive enough to capture the novel concept \todo{cite-Lora,cite-OGD,more?}.
Specifically, we make the assumption that the restricted parameterization can still optimize the customization loss very well:
\begin{assumption}\label{assumption:projected}
% \begin{align*}
$
    \forall i, \min_\theta \lL_i(\theta) \approx \min_\Theta \lL_i(\theta_o + B_i\Theta).
$
% \end{align*}.    
\end{assumption}
% This assumption makes sense due to over-parameterization of the network.
\todo{Figure~\ref{fig:constrained-optimization} provides some empirical evidence showing that even in the constrained space, we can achieve results that are un par in quality with optimizing the full space.}
\input{figures/constraint-cus/fig}


\begin{figure*}[t!]
    \centering
\includegraphics[width=\linewidth]{figures/experiments/PLACEHOLDER_identity_preservation.png}
    \caption{\textbf{Identity Preservation}}
    \label{fig:enter-label}
\end{figure*}

% Under this formulation, we will have the following theorem:

\subsection{\todo{Instant Concept Fusion}}
\guandao{
1. if we can allow training sequential merging the concepts, then we can do the continue learning without knowing the datasets
2. but this is not scalable as we want instant concept merging without optimization
3. We made this assumptions (observation). describe in texts preferred
4. then we allow decentralized training AND scalable merging. 
}
With the weights optimized as indicated by Equation~\ref{eq:projected-sgd}, we propose to create merge weights in the following way:
\begin{align}
    \theta_{\text{merge}} = \theta_o + \sum_i \lambda_i (\theta_i^* - \theta_o),
\end{align}
where $\lambda_i$ is the weighted for the concept $i$ and $\theta^*_i$ is the optimal weights created through Equation~\ref{eq:projected-sgd}.
Intuitively, $\theta_i^*-\theta_o$ aggregates all gradient updates of the form: $\sum_t \theta_i^{t+1} - \theta_i^t$. 
\todo{(connect back to orthogonal gradient descent).}
But this is different from orthogonal gradient descent as the updating step is taking from $\theta_o$ instead of $\theta_i^*$.
However, the fine-tuning result of $\theta_i^*$ is usually very close to $\theta_o$ \todo{cite?}.
This allows us to make the following assumption that locally the gradient of loss $\lL_i$ remains roughly unchanged when evaluated at a different point with translation orthogonal to the basis $B_i$:
\begin{assumption}\label{assumption:grad}
$\nabla_\theta \lL_i(\theta_o + B_i\Theta_i + B_j\Theta_j)$ is approximately the same as
$\nabla_\theta \lL_i(\theta_o + B_i\Theta_i)$ for all $i \neq j$.
\end{assumption}
\todo{With the combination of assumption~\ref{assumption:grad} and assumption~\ref{assumption:projected}, we are able to show that the $\theta_{\text{merge}}$ is equivalent to doing orthogonal gradient descent. (still need to rephrase this).}


\subsection{Generating Orthogonal Bases $B_i$'s}

A key challenge of the method described in previous sections is to generate a set of bases $B_i$ that are orthogonal to each other.
Note that this is very difficult especially because when choosing basis $B_i$, the user is not aware of what basis the other users chosen to optimize for the concepts to be combined in the future.
Strictly enforcing such orthogonality might be infeasible without prior knowledge of other tasks.
We instead propose a relaxation to the constraint, introducing several methods to achieve approximate orthogonality.

\paragraph{Randomized orthogonal basis.}
One method for enforcing approximate orthogonality is achieved by determining a common basis.
For some linear weight $\theta \in \Re^{m\times n}$, we first generate a large orthogonal basis $O\in \Re^{n\times n}$. This orthogonal basis is shared between all users. During training of concept $i$, $B_i$ is formed from taking a random subset of $k$ columns from $O$. Given $k \ll n$, the probability of two randomly chosen $B_i$'s to share the same columns is kept low. In the case of 


\paragraph{Randomized gaussian.}
Specifically, we sample each entry of $B_i$ from a zero-mean gaussian with standard deviation $\sigma$: $B_i[k] \sim \nN(0, \sigma^2 I)$.
When the dimensionality of $B_i$ is high, this simple strategy creates matrices that are orthogonal in expectation: $\Ee\left[B_i^TB_j \right] = 0$ \todo{cite?}.
\todo{should we explain a bit here?}
\todo{I can also see some alternatives, such as construct a orthogonal basis. should we consider them?}
The advantage of







\subsection{Implementation Considerations}
\input{figures/method/fig}


==> sec/3_method_fedavg.tex <==
\section{Method}\label{sec:setup}
\input{figures/problem-setup/fig}
% \kac{It's weird to see the following part in the related work section, maybe let's convert it into a short background subsection within the method section that covers the customization of $\Delta \theta$ and federated averaging? }
% \todo{Po: introduce core equations for customization}

In this section, we first introduce the problem setting of modular customization (Sec.~\ref{sec:mod-cus}). We then take a look at the simple solution of Federated Averaging~\cite{mcmahan2023communicationefficient}, and explore where and why this naive method fails (Sec.~\ref{sec:fedavg}). Motivated by the limitations of Federated Averaging, we discuss the conditions to ensure concept identity preservation (Sec.~\ref{sec:preserve}), and finally introduce our solution to modular customization -- \textbf{\textit{orthogonal adaption}} (Sec.~\ref{sec:orth-adapt} and Sec.~\ref{sec:basis}).

\subsection{Modular Customization}\label{sec:mod-cus}
In this paper, we are interested in customizing text-to-image diffusion models to generate multiple personal concepts in an efficient, scalable, and decentralized manner. 
%We refer to such a task as \textbf{\textit{modular customization}}, as individual fine-tuned models should act like independent modules, which can be combined with others in a plug-and-play manner without additional training.
In a single-concept customization setting, each user is able to create their own customized concepts by defining a set of images $\iI^i = \{I^i_j\}_j$. A diffusion model is then fine-tuned, optimizing model parameters and corresponding text embeddings to reconstruct the target images using the diffusion loss (Eq.~\ref{eq:diff-loss}). However, in addition to single-concept text-to-image customization, users are usually interested in seeing multiple personalized concepts interacting together.
This calls for a text-to-image model that is aware of a set of customized concepts.
Being able to generate multiple personalized concepts in a single model, however, is challenging.
First, all possible sets of concepts is growing exponentially with respect to the number of personal concepts, which is only going to be an ever-increasing number. 
As a result, it's important for personalized concepts to be merged with interactive speed.
Furthermore, users usually have limited compute at their end (\eg a phone or a personal laptop without SOTA GPUs), which means any computation done on the users end should ideally be trivial.

These requirements motivate an efficient and scalable fine-tuning setting we call \textbf{\textit{modular customization}}, where individual fine-tuned models should act like independent modules, which can be combined with others in a plug-and-play manner without additional training. The setting of modular customization involves three stages: individual fine-tuning, merging of concepts and multi-concept generation. Fig.~\ref{fig:setup} provides an illustration of this three stage process.

With modular customization in mind, our goal is to design a fine-tuning scheme, such that individually fine-tuned models can be trivially combined (e.g. summation) with any other fine-tuned model to enable multi-concept generation. 
%An important constraint to this setting is that each individual user is unaware of other concepts during their own fine-tuning process. Therefore, a solution to modular customization should produce models that can be combined with any other model fine-tuned under the same regime.



\subsection{Federated Averaging}\label{sec:fedavg}
Perhaps the most straight-forward but effective technique for achieving modular customization is to take a weighted average of each individually fine-tuned model. This technique is often referred to as Federated Averaging (FedAvg)~\cite{mcmahan2023communicationefficient}. Given a set of learned weight residuals $\Delta\theta_i$ optimized on concept $i$. The resulting merged model is simply given by,
\begin{equation}
    \theta_{\text{merged}} = \theta + \sum_i \lambda_i\Delta\theta_i,
\end{equation}
where $\theta$ represents the pre-trained parameters of the model used for fine-tuning, and $\lambda_i$ is a scalar representing the relative strength of each concept. While federated averaging is fast and places no constraints on the expressivity of each individually fine-tuned model, naively averaging these weights can lead to loss of subject fidelity due to interference between the learned weight residuals. This effect is especially severe when training multiple semantically similar concepts (e.g. human identities), as learned weight residuals tend to be very similar. We coin this undesirable phenomenon "crosstalk".
Our approach is inspired by FedAvg.
We adopt its computational efficiency but modify the fine-tuning process to ensure  minimal interference between learned weight residuals between different concepts.
We want to enable instant, multi-concept customization from individually trained models without sacrificing subject fidelity.

\subsection{Preserving Concept Identity}\label{sec:preserve}
With the goal of addressing the limitations of federated averaging, we first examine where this method fails. For simplicity, consider the case of merging two concepts $i$ and $j$. After fine-tuning on each individual task, we receive a set of learned weight residuals $\Delta\theta_i$ and $\Delta\theta_j$. The output of a particular linear layer in the fine-tuned network is
%
\begin{equation}
    O_i = (\theta + \Delta\theta_i)X_i,
\end{equation}
%
where $X_i$ represents a particular input to the layer corresponding to the training data of concept $i$. 
%Our goal is to construct $\Delta\theta_j$ such that the value of $O^l_i$ is preserved even after merging. Consider the simple case of federated averaging with $\lambda = 1$. The resulting merged model produces,
When merging the two concepts using federated averaging with $\lambda = 1$, the resulting merged model produces
%
\begin{equation}
    \hat{O}_i = (\theta + \Delta\theta_i + \Delta\theta_j)X_i.
\end{equation}
%
Note that, without enforcing specific constraints, it is likely that this leads to $\Delta\theta_jX_i\neq0$ and, subsequently, $\hat{O}_i \neq O_i$.

\begin{claim}
A concept $i$ is preserved \ka{in a customized model merged with other customized weights through federated averaging} if the row space of the learned residuals $\Delta\theta_i$ is orthogonal to the column space of the layer inputs $X_j$ \ka{for every concept} $j \neq i$.
\end{claim}

It can be observed that the mapping of data for concept $i$ is preserved when $\Delta\theta_j X_i = 0$ \ka{for $j \neq i$}. By symmetry, the mapping of data for concept $j$ is preserved given $\Delta\theta_i X_j = 0$ \ka{for $i \neq j$}. The challenge of concept preservation then comes from designing $\Delta\theta_i$ and $\Delta\theta_j$ such that the orthogonality condition is satisfied. Note that given enough data for training a certain concept $i$, $X_i$ is likely to have full column rank. This makes the orthogonality condition impossible to satisfy. We propose to impose a relaxation of this constraint, choosing to $\minimize||\Delta\theta_i X_j||$ instead. Intuitively, $||\Delta\theta_i X_j||$ measures the amount of crosstalk between concept $i$ and $j$. We would like to keep this value low to ensure subject identity is preserved even after merging.


\subsection{Orthogonal Adaptation}\label{sec:orth-adapt}
Motivated by the objective of minimizing $||\Delta\theta_i X_j||$ while keeping $||\Delta\theta_i X_i||$ non-zero, we propose \textit{\textbf{orthogonal adaptation}}. Similar to low-rank adaptation (LoRA), we represent learned weight residuals through a low-rank decomposition of the form

%
\begin{equation}
    \Delta \theta_i = A_iB_i^T, \theta_i\in\Re^{n\times m} A_i\in\Re^{n\times r}, B_i\in\Re^{m\times r},
\end{equation}
%
where the rank $r <\!\!< \min(n,m)$. However, contrary to conventionally fine-tuning with LoRA, we keep $B_i$ constant, and only optimize $A_i$. 
\input{figures/method/fig}

In order to minimize $||\Delta\theta_jX_i||$, we define the columns of $B_j$ as a set of random vectors in $\Re^m$. Since $B_j$ is low rank by definition, we expect $||\Delta\theta_jX_i||$ to be small, as we are taking the projection of $X_i$ into a small $k$ dimensional subspace 
%\kac{The fact that we project something into a low dimensional space, doesn't mean that the magnitude of the projection is small, right? Only in case that they are nearly orthogonal, but I didn't see such a claim that justifies that they are orthogonal} \po{I think the idea here is that since $k<<m$ and that the columns of $B_i$ are randomly chosen, the projection is expected to be much smaller in comparison to the original.}
. Conversely, $B_i$ is also chosen in a similar manner to minimize $||\Delta\theta_iX_j||$.

However, naively choosing $B_i$ and $B_j$ will lead to poor results. This is because we expect the learned residuals for a concept to have meaningful interactions with their data, and therefore assume $||\Delta\theta_iX_i||$ to be non-zero. Specifically, we want the components of $X_i$ that are preserved after merging to have non-trivial interactions with $\Delta\theta_i$ to ensure identity preservation. Given $\Delta\theta_j = A_jB_j^T$, components of $X_i$ that lie in the orthogonal complement of $B_j$ are preserved. Referring to this orthogonal subspace as $\bar{B_j}$, we wish to design $B_i$ such that $||\Delta\theta_i\bar{B_j}|| = ||A_iB_i^T\bar{B_j}||$ is non-trivial. One (sufficient but not necessary) way of satisfying this condition is to enforce $B_i^TB_j = 0$. This condition ensures that the columns of $B_i$ would lie in the orthogonal complement of the column space of $B_j$, causing $B_i^T\bar{B_j}$ to be non-trivial, and therefore $||\Delta\theta_i\bar{B_j}||$ to also be non-trivial.

% In order to satisfy the orthogonality constraint $\Delta\theta_jS^l_i = 0$, we define the columns of $B_j$ as a set of orthogonal vectors. Given $B_j$ is low rank, the orthogonal complement of the column space of $B_j$ still spans most of $\Re^m$, providing a good candidate for $S^l_i$. We therefore define $S^l_i = \bar{B_j}$, where the columns of $\bar{B_j}$ spans the desired orthogonal complement \guandao{Do you mean $span\{S_i^j\}\subseteq span\{B_j\}, \forall i \neq j$?}. Conversely, defining $B_i$ and $S^l_j$ in a similar manner provides us with a sufficient condition for satisfying the orthogonality objective.

% \paragraph{Choosing $B_i$.} Naively choosing $B_i$ and $B_j$ will lead to poor results. This is because we expect the learned residuals for a concept to have meaningful interactions with their data, and therefore assume $||\Delta\theta_iS^l_i|| >\!\!> 0$. Substituting our definition for $\Delta\theta_i$ and $S^l_i$ gives,
% \begin{equation}
%     ||A_iB_i^T \bar{B_j}|| >\!\!> 0.
% \end{equation}
% From this, we expect $B_i^T \bar{B_j}$ to be non-zero. One way of satisfying this condition is to enforce $B_i^TB_j = 0$. \guandao{Why we need $B_i^TB_j=0$ to have $B_i^T\bar{B}_j = 0$?} Intuitively, this means that the columns of $B_i$ should lie in the orthogonal complement of the column space of $B_j$.

\paragraph{Expressivity of orthogonal adaption.} Expressivity of our method arises as a natural concern. As we are optimizing significantly less parameters by freezing $B$. Fortunately, text-to-image diffusion models are often over-parameterized, with millions/billion of parameters. Prior works have shown that even fine-tuning a subspace of such parameters can be expressive enough to capture the novel concept. We also show this result empirically in Fig.~\ref{fig:constrained-optimization}, where our method leads to results with similar fidelity, even without the need to optimize $B$ during training.

\input{figures/constraint-cus/fig}

\subsection{Designing Orthogonal Matrices $B_i$'s}\label{sec:basis}
A key challenge of the method described in previous sections is to generate a set of basis matrices $B_i$ that are orthogonal to each other.
Note that this is very difficult especially because when choosing $B_i$, the user is not aware of what basis the other users chosen to optimize for the concepts to be combined in the future.
Strictly enforcing such orthogonality might be infeasible without prior knowledge of other tasks.
We instead propose a relaxation to the constraint, introducing a simple and effective method to achieve approximate orthogonality.

% \paragraph{Randomized orthogonal basis.}
One method for enforcing approximate orthogonality is to determine a shared orthogonal basis.
For some linear weight $\theta \in \Re^{m\times n}$, we first generate a large orthogonal basis $O\in \Re^{n\times n}$. This orthogonal basis is shared between all users. During training of concept $i$, $B_i$ is formed from taking a random subset of $k$ columns from $O$. Given $k <\!\!< n$, the probability of two randomly chosen $B_i$'s to share the same columns is kept low.

% \paragraph{Randomized Gaussian Matrices.}
% Another method that enforces approximate orthogonality is to simply draw entries in $B_i$ from a zero-mean distribution. Specifically, we sample each entry of $B_i$ from a zero-mean Gaussian distribution with standard deviation $\sigma$: $B_i[k] \sim \nN(0, \sigma^2 I)$.
% When the dimensionality of $B_i$ is high, this simple strategy creates matrices that are orthogonal in expectation: $\Ee\left[B_i^TB_j \right] = 0$ \todo{cite?}.

\subsection{Implementation Details}

==> sec/3_method_v0.tex <==
\section{Problem Set-up}
In this paper, we are interested in creating composible customized concepts in text-conditioned diffusion models.
Specifically, each user is able to create their own customized concepts by defining a set of images $\iI^i = \{I^i_j\}_j$ and a special token $t_i$ that identifies the common object inside the dataset  $\iI_i$.
Our algorithm aims to predict an embedding for the identity token (i.e. $c_i$) and a set of weights update $\Delta \theta_i$ for the diffusion model.
\todo{(wording):}
These weights $\Delta \theta_i$ are obtained by optimizing two objectives:
1) mapping $t_i$ to corresponds to the common object in $\iI_i$;
2) preventing the customized model (i.e. when using weight $\theta + \Delta \theta_i$) to catastrophically forget already learned information; and last but not least
3) these concepts $c_i$ and $\Delta \theta_i$ can be combined with different concepts, e.g. $c_j, \Delta \theta_j$ with minimum additional computation.
The goal is to enable the decentralized creation of customized concepts that can be composed together with minimal effort.

\section{\todo{Mathematical Formulation}}
We follow ~\todo{Dreambooth} to achieve these goals to optimize $\theta_i$ for the following objectives.

First, we would like to ensure that the finetuned weights can generate images in $\iI_i$ when using $c_i$ in the caption.
This can be achieved by optimizing the customization loss:
\begin{align}
    \label{eq:loss-cus}
    \lL_{\text{cus}}(\theta,\iI_i, c_i) = \Ee_{x\sim \iI_i,t,\epsilon}\left[
        \norm{
        \mM_{\theta}\paren{x_t, t, c_i} - x
        }^2
    \right],
\end{align}
where $\mM$ is the diffusion model,
$\mM$ is the diffusion model,
$x_t = \alpha_t x + \beta_t \epsilon$ with $\epsilon\sim\nN(0,I)$ is the Gaussian noise, 
$\alpha_t, \beta_t$ are weights schedules \todo{cite-EDM}.
This loss makes sure the fine-tuned diffusion model can generate images containing the subject the concept $c_i$ wants to capture while conditioned on the customized caption.

\todo{Regularization loss might not be explicit (try to remove it)}
Optimizing loss in Equation~\ref{eq:loss-cus} alone can lead to the model catastrophically forgetting \todo{(wording)}. 
To prevent this from happening, \todo{Dreambooth} suggest the following loss:
\begin{align}
\lL_{\text{reg}}(\theta,\dD)
=
\Ee_{(x,c)\sim\dD,t,\epsilon}\left[
        \norm{
        \mM_{\theta}\paren{x_t, t, c} - x
        }^2
    \right],
\end{align}
where $\dD$ is a dataset generated by using the original weight $\theta$ and a set of captions.
In Dreamboth~\cite{dreambooth}, this set of regularized captions usually contains the class label for the customized concept.
\todo{Different papers make different choices of selecting these regularization captions.}

Users are interested in combining these customized concepts into the same model.
To find the parameter $\theta$ for multiple concepts with data $\iI_i, c_i, \dD_{\text{reg}}$, one can optimize customized loss for all data:
\begin{align}
    \lL(\theta) = \lL_{\text{reg}}(\theta,\dD_{\text{reg}})+ \sum_{i} \lambda_i\lL_{\text{cus}}(\theta,\iI_i, c_i).
\end{align}
However, such optimization can be computationally expensive to run for each possible combination of concepts. 
\todo{other potential performance issue?}
In this paper, we propose a method to customize the weights for the diffusion models (i.e. finding $\theta_i$) that can be combined together without any additional fine-tuning/optimization.


\section{Method}
\label{sec:method}
\todo{guandao: talk about the gradient objectives}
In this section, we will describe our method to achieve decentralized yet compositionable customization efficiently.
The key idea is to construct update weights $\Delta \theta_i$ that are orthogonal to different concepts $c_j$ (i.e. $i\neq j$).
We will first introduce how do we construct the finetuning parameters in Sec~\ref{sec:params}.
We then show that \todo{how our construction can preserve optimality of the loss even if optimized independently}.

\subsection{Training Parameters}
\label{sec:params}
Diffusion models use the following attention layer to modulate visual features using language features:
% \begin{align}
%     \operatorname{attn}(\ff_q, \ff_k) = \operatorname{Softmax}
%     \underbrace{\paren{
%         (W^q\ff_k)^T(W^k\ff_k)^T
%     }}_{n\times m}
%     \underbrace{(KW^v)^T}_{m \times d_o}
% \end{align}
\begin{align*}
    \operatorname{Attn}(Q, C) = \operatorname{Softmax}
    \paren{
        \frac{Q(W^q)^TW^kC^T}{\sqrt{d_o}}
    }
    (W^vC^T)
\end{align*}
where $Q\in\Re^{n\times d_q}$ is the visual features and $C\in\Re^{m\times d_k}$ is the text features.
$W_q\in \Re^{d_a\times d_q}$, $W_k \in \Re^{d_a\times d_k}$, and $W^v \in \Re^{d_o \times d_a}$ are linear layer weights for queries and values.
% $d_q$ is the dimension for the queries (visual features).
% $d_k$ is the dimension for the keys (language features).

Following \todo{cite-custom-diffusion}, it's usually sufficient to only fine-tune the parameters interacting with the word embedding: $W^v$ and $W^k$.
For each cross-attention layer, we will create a fine-tuning weight for each concept $c_i$ in the following form:
\begin{align*}
    \Delta W^k = L^kR_i,\quad 
    \Delta W^v = L^vR_i,
\end{align*}
where $R\in\Re^{r\times d_q}$ is a set of orthonormal basis (i.e. $RR^T$)$L^{k,v}\in\Re^{d_a\times r}$ are parameters we will optimize.
\todo{When $r$ is small, this is a low-rank approximation. what's the best way to bring this in?}
The customized attention weight for the $i^{\text{th}}$ concept will be :
\begin{align*}
    W^k_i = W^k + \Delta W^k_i \quad 
    W^v_i = W^v + \Delta W^v_i,
\end{align*}
where $W^k$ and $W^v$ are the original weights of the diffusion model.
To obtain $W^k_i$ and $W^v_i$, we can optimize $\lL_{\text{cus})}$ and $\lL_{\text{reg}}$ for the concept using dataset $\iI_i, c_i$, similar to \todo{custom diffusion single-concept training.}


\subsection{Efficient Multi-concept Merging}
How do we fuse different concepts together without retraining?
One simple way to achieve this is to sum different residual $\Delta W^{k,v}_i$ together to obtain the merged weights:
\begin{align*}
    W^{k,v}_m = W^{k,v} + \sum_i \Delta W^{k,v}_i.
\end{align*}
However, since these weights are fine-tuned on individual concepts \todo{without knowing the need to merge with the others.}
Such failure case has been observed by several prior works \todo{cite}.

To prevent such failure case from happening, we would like to make sure that $\Delta W_i$ does not interact with $c_j$ whenever $i \neq j$.
Specifically, we want:
\begin{align*}
    i\neq j \implies \Delta W^{k,v}_i c_j = 0.
\end{align*}

We can have the following theorem:
\begin{theorem}
Let $W^{k,v}_i$ be the set of weights that optimize $\lL_{\text{cus}}(\cdot, \iI_i, c_i)$, and $\forall i\neq j, \Delta W^{k,v}_i c_j = 0$, then $W^{k,v}_m$ that minimizes $\sum_i \lL_{\text{cus})}(\cdot, \iI_i, c_i)$.
\end{theorem}
Please refer to the supplementary for the proof.

\subsection{Orthogonality}
How do we achieve $\forall i\neq j, \Delta W^{k,v}_i c_j = 0$? 
We propose to do that by enforcing the following two constraints:
\begin{align}
\forall i\neq j,
R_i c_j  =0, \quad R_i c_i \neq 0
\end{align}
This can be achieved by \todo{how do we implement it?}

It's easy to show that this implies $\Delta W_i^{k,v}c_j = 0$:
\begin{align}
    \Delta W_i^{k,v} c_j = L^{k,v}R_i c_j = L^{k,v} 0 = 0.
\end{align}


\todo{IGNORE THE REST.}
Preserving the loss for regularization
\begin{align}
\begin{cases}
    X (C_r W_m^k)^T = X(C_r W^k)^T, \forall X \in \Re^{n \times d_a} \\
    X (C_r W_m^v)^T = X(C_r W^v)^T, \forall X \in \Re^{n \times m}
\end{cases}
\end{align}
which implies
\begin{align}\label{eq:detal-reg-opt}
\begin{cases}
    C_r \Delta W_i^k = 0,\ \forall i \\
    C_r \Delta W_i^v = 0,\ \forall i
\end{cases}.
\end{align}
which will be the condition that makes $\mathcal{L}_{reg}=0$.

Similarly, preserving the optimality of the customization loss, it's sufficient that
\begin{align}
\begin{cases}
    X (c_i W_m^k)^T = X(c_i W^k_i)^T, \forall X \in \Re^{n \times d_a}, \forall i \\
    X (c_i W_m^v)^T = X(c_i W^v_i)^T, \forall X \in \Re^{n \times m}, \forall i
\end{cases},
\end{align}
which implies 
\begin{align}\label{eq:detal-cus-opt}
\begin{cases}
    c_i \Delta W_j^k = 0,\ \forall i \neq j\\
    c_i \Delta W_j^v = 0,\ \forall i \neq j
\end{cases}.
\end{align}

\subsection{Low-rank Approximation to enforce Customization Loss Optimality}

One way to enforce the conditions in Equation~\ref{eq:detal-cus-opt} and Equation~\ref{eq:detal-reg-opt} is to construct the low-rank approximation and enforce orthogonality.
First, construct low rank approximation for $\Delta W_i^k$ and $\Delta W_i^v$ in the following way:
\begin{align}
\begin{cases}    
    \Delta W_i^k &= L_i^T D_i^k R_i^k \\
    \Delta W_i^v &= L_i^T D_i^k R_i^v
\end{cases}
\end{align}
where 
$L_i^{k,v} \in \Re^{l_i \times d_k}$,
$D_i^{k,v} \in \Re^{l_i \times r_i}$,
and 
$R_i^{k,v} \in \Re^{r_i \times d_a}$.
\todo{NOTE: we can combine $D_i^{k,v}R_i^{k,v}$ into the same matrix of shape $\Re^{l_i\times d_a}$ that is optimizable.}

Then we enforce the concept vector $c_i$ to live in the basis provided by $L_i$:
\begin{align}
    c_i = \alpha_i^T L_i,
\end{align}
\todo{NOTE: needs to share the basis $L_i$ for both values and keys.}
$\alpha_i\in \Re^{1\times l_i}$ are the coefficients for the concept in basis $L_i$.

Given this construction, we have:
\begin{align}
    \forall i \neq j,\ L_iL_j^T = \mathbf{0} 
    \implies 
    \forall i \neq j,\ c_i \Delta W_j^{k,v} = \mathbf{0}
\end{align}
because
\begin{align}
c_i\Delta W_j^{k,v}
&= \alpha_i^T L_i L_j^T D_j^{k,v} R_j^{k,v}\\
&= \alpha_i^T \mathbf{0} D_i^{k,v} R_j^{k,v} = \mathbf{0}
\end{align}

\todo{NOTE: this our previous reasoning, which enforce the wrong constraints}
\begin{align}
    \forall i\neq j, R_iR_j^T=\mathbf{0} 
    \implies
    \forall i\neq j, (C_r\Delta W_i)^T(C_r\Delta W_j) = 0
\end{align}


\todo{IDEA: choose $L_i$ from the null space of $C_r$}
Assume $C_r\in \Re^{n\times d_k}$ has the following SVD: 
\begin{align}
    C_r = \begin{bmatrix}
    U_r\ U_n
    \end{bmatrix}\begin{bmatrix}
    S_r\ &\mathbf{0} \\
    \mathbf{0}\ &\mathbf{0} 
    \end{bmatrix}\begin{bmatrix}
    V_r \\
    V_n
    \end{bmatrix}
\end{align}
then choosing $L_i \subset V_n$ can enforce Equation~\ref{eq:detal-reg-opt}.
This is because  $C_rL_i^T = 0$.
But this can be difficult if $n > d_k$.

